A Technical Review of Wireless security for the Internet of things: Software Defined Radio perspective

The increase of cyberattacks using IoT devices has exposed the vulnerabilities in the infrastructures that make up the IoT and have shown how small devices can affect networks and services functioning. This paper presents a review of the vulnerabilities of the wireless technologies that bear the IoT and assessing the experiences in implementing wireless attacks targeting the Internet of Things using Software-Defined Radio (SDR) technologies. A systematic literature review was conducted. The types of vulnerabilities and attacks that can affect the wireless technologies that stand the IoT ecosystem and SDR radio platforms were compared. On the IoT system model layer, perception layer was identified as the most vulnerable. Most attacks at this level occur due to limitations in hardware, physical exposure of devices, and heterogeneity of technologies. Future cybersecurity systems based on SDR radios have notable advantages due to their flexibility to adapt to new communication technologies and their potential for the development of advanced tools. However, cybersecurity challenges for the Internet of Things are so complex that it is needed to merge SDR hardware with cognitive techniques and intelligent techniques such as deep learning to adapt to rapid technological changes.

==> A Technical Review of Wireless security for the Internet of things_/1_introduccion.tex <==
On September 5 and 6, 2019 a cyber-attack affected several Wikipedia sites in Europe - including  Germany, France,Italy and Poland, at the same time as parts of the Middle East \cite{Bankinfosecurity2019}.IoT devices were used to take down Wikipedia through distributed denial of service (DDoS) attacks. The IoT were used to amplifying the potential cyberattack surface.According to the World Economic Forum report, attacks on IoT devices grew by more than 300\% in the first half of 2019 \cite{Weforum2020},\cite{Kaspersky2019}.

On May , 2018 the VPNFilter malware targets at least 500K networking devices  in 54 countries \cite{Enisa2018}. Home-office network devices, as well as network-attached storage devices were infected. VPNFilter exploited various vulnerabilities in several models and brands of routers and network-attached storage (NAS) devices.
%The malware can persist even if the infected device is rebooted. 
The malware capabilities identified including data exfiltration, spying on traffic, and rendering the infected device unbootable. The malware code overlaps with versions of the BlackEnergy malware, which was responsible for multiple large-scale attacks that targeted devices in Ukraine.

%One of its more troubling actions is the interception of the Supervisory Control and Data Acquisition (SCADA) protocol communications used by much industrial plant machinery.

%Devices brands as Linksys, MikroTik, Netgear, and TP-Link,ASUS, D-Link, Huawei, Ubiquiti, UPVEL, and ZTE were nfected.

%are ASUS, D-Link, Huawei, Ubiquiti, UPVEL, and ZTE. New devices were also discovered from Linksys, MikroTik, Netgear, and TP-Link.

%infecting Ukrainian hosts at an alarming rate, utilizing a command and control (C2) infrastructure dedicated to that country.  

%One of its more troubling actions is the interception of the Supervisory Control and Data Acquisition (SCADA) protocol communications used by much industrial plant machinery.


%VPNFilter exploited various vulnerabilities in several models and brands of routers and network-attached storage (NAS) devices. Trend Micro’s research also revealed that the devices, including IP cameras and printers, weren’t just susceptible to VPNFilter, but to other publicly known security flaws — and in turn, a host of other attacks, such as remote code execution, command injection, and information leak/disclosure among others.

%VPNFilter is notable in that it can persist even if the infected device is rebooted.

On April 7, 2017, a cyberattack on the emergency system in the city of Dallas, in the United States, triggered 156 emergency sirens at 11:40 p.m., causing panic and fear of a possible terrorist attack \cite{WIRED2017}.The case study carried out by the company Bastille Networks \cite{BalintSeeberBastille2018}, found that the attacker exploited the vulnerability of the wireless infrastructure making up the emergency system to control its operation and also found that the United States has over 5000 similar emergency systems distributed throughout different cities, universities, military facilities and industries.

On October 21, 2016 \cite{DYN2016}, a denial-of-service cyber-attack targeting Internet provider DynDNS caused problems for sites such as Twitter, Netflix, Spotify, Airbnb, Reddit, Etsy, SoundCloud and the New York Times, affecting much of the United States of America. According to subsequent analyses \cite{Securityintelligence},thousands of IoT devices such as cameras and home routers were used, which were violated in various ways. The traffic volume of this attack has been the highest recorded so far: 1.2 Tbps; a similar event recorded previously had reached 620 Gbps.


These security incidents are an exemplify the vulnerability of some of today's communication systems. At a point in history where society is moving rapidly towards technological scenarios supported largely by the Internet of Things (IoT) communications infrastructure \cite{Gupta2015}, such threats represent a global challenge. 

The International Telecommunication Union estimates 25 billion connected devices for 2020 \cite{ITU2016}; and according to the Ericsson mobility report \cite{Ericcson2017} by 2022 the number of connected devices will be 29 billion, with a projected increase of 21\% between 2016 and 2022.\cite{Stellios2018} identifies potentially vulnerable scenarios and describes risks in critical infrastructure such as power distribution, SCDA, smart transport, medical care and smart home automation. When analyzing the technological infrastructure that supports the IoT \cite{Zayas2017}, we find a diverse ecosystem of wireless technologies, with rapid growth and some gaps in the regulation of device-manufacturing processes.

Risk assessment and analysis of the impact of cyberattacks is a concern that goes beyond technical and academic scenarios. The OECD (Organisation for Economic Cooperation and Development), in its Recommendation on Digital Security Risk Management for Economical and Social Prosperity \cite{Economy2015}, analyses the issue of digital security and its impact on the economic development of countries.\cite{E&Y2015} estimates that 70\% of connected IoT devices have vulnerabilities.  \cite{CommitteeonScienceSpace} analyses the risks and the ways in which such events can affect the operation of vital systems for people. In 2014, it was estimated that the economic impact of cybercrime was 500 billion dollars. By 2018, this figure had reached 600 billion \cite{Lewis2018}.In 2021,cybercrime damages might reach US\$6 trillion \cite{Weforum2020}.

Some Governments, concerned about threats to their communications infrastructures, have created special programs to counter them. The United States government through the Advanced Research Projects Agency (DARPA) created the Trusted Integrated Circuits program to develop technologies that ensure reliability in the manufacturing processes of electronic devices used in military systems. Other countries are undertaking similar initiatives through cyber security agencies such as Agence nationale de la sécurité des systèmes d'information (ANSSI) in France; Nationales Cyber-Abwehrzentrum in Germany; and Defence Cyber Operations Group in the United Kingdom.

A large part of IoT technologies are wireless and form an ecosystem of radios designed from various communication protocols \cite{Frustaci2018}. The old radio systems required specific hardware to operate in a very limited range of frequencies \cite{Mitola1999}. Modern radios are evolving towards Software-defined radio technology (SDR), where the same hardware platform can adapt and become a transmitter and/or receiver system operating under various technologies, by modifying the software's configuration parameters in the device. Although the development of ADC-DAC converter manufacturing techniques and FPGA-based processing systems have led to significant improvements in hardware performance, there are still several technical limitations to the production of the ideal SDR radio device proposed by Joseph Mitola in 1999 \cite{Mitola1999}. \cite{Pawelczak2011} presents an analysis of the first ten years of SDR technology development, while \cite{Mitola2015}  describes the evolution of trends in SDR considering the last two decades.

The large growth of wireless devices for IoT development also causes risks and vulnerabilities to increase. The types of wireless attacks are varied and there is no single classification. Among the best known are: spoofing, eavesdropping, sidechannel, jamming, replay and spoofing. All of them are based on exploiting the various vulnerabilities present in radio devices or in their communication protocols.

The review made allows, firstly, to clarify the dimension of the wireless ecosystem of the IoT, with its technologies and protocols, and then the concepts related to radio technology defined by software and the types of existing hardware and software resources, as well as their characteristics and technical possibilities. It then addresses the concepts of wireless cybersecurity, in order to finally identify the types of vulnerabilities and attacks that can affect the wireless technologies that make up the IoT ecosystem SDR radio platforms and cognitive radio networks. In the document, the security aspects related to SDR technology are analyzed in two ways: first by identifying the vulnerabilities inherent to SDR devices since the flexibility and reconfigurability of SDR hardware make its adaptability very high, but they can also be affected by attacks capable of modifying radio behavior. This aspect is very important for the future of wireless systems, where cognitive radio networks will be supported by reconfigurable radios. The second aspect considered in the review was the classification of various experiences in implementing wireless attacks using commercial SDR radios, and the use of these platforms as tools for the analysis of risks and vulnerabilities in wireless systems. The contributions of the review are the following:

\begin{itemize}[]
    \item Classifying and identifying the technologies that make up the wireless ecosystem of the Internet of Things, their standards and operating frequencies.

    \item Contextualizing definitions and concepts related to SDR technology and the various hardware architectures.

    \item Classifying the most common SDR hardware platforms considering their main technical characteristics.

    %\item Descripción de los  ciberseguridad
    \item Identifying the types of SDR radios and cognitive radio networks vulnerabilities.
    
    \item Identifying the most common types of wireless vulnerabilities and IoT wireless ecosystem vulnerabilities.
    
    \item Understanding wireless attack implementation experiences and vulnerability assessments for wireless technologies, and identifying the types of SDR radio platforms used.
\end{itemize}

The document is organized as follows: section two presents the context of the technologies that make up the wireless ecosystem of the Internet of Things, their operating frequencies and standards. Thereafter, section three includes definitions of concepts related to software-defined radio, the types of hardware architectures and a technical comparison of the most commonly used SDR platforms. 
%It also includes a description of the technical characteristics of USRP platforms, daughterboards, communication protocols and software tools. The fourth section includes the definition of cognitive radio. 
The fourth section addresses issues related to wireless cybersecurity. This includes classifying SDR radio vulnerabilities, common wireless vulnerabilities, and IoT wireless ecosystem vulnerabilities and cognitive radio network vulnerabilities. This section also describes various experiences in wireless attacks and wireless security deployments, and the analysis performed using software-defined radio platforms. Experiences are identified and classified according to the types of attacks implemented and SDR platforms used are described. Finally, section five includes an analysis on the most significant elements identified from the review process carried out.




==> A Technical Review of Wireless security for the Internet of things_/2_ecosistema.tex <==
\begin{figure*}[ht!]
        \centering
        \caption{Ecosystem of wireless technologies used for the IoT. Based on \cite{KeysightTechnologies2019}, Fig 2}
        \includegraphics[width=1\textwidth]{images/Ecosystem.pdf}
        \label{fig:ecosistema}
\end{figure*}

Figure \ref{fig:ecosistema} shows a classification based on \cite{KeysightTechnologies2019} for some of the wireless communication technologies used in the implementation of the Internet of Things, taking into account the range of their scope. By classifying wireless technologies by range, we can talk about technologies: of proximity, WPAN, WFAN, WLAN, WNA and WWAN.



The frequency bands for the operation of each can be appreciated, along with the corresponding standards. This technological scenario considers the technologies existing in 2019 and their evolution towards a 5G technologies-based future ecosystem. \cite{Yang2018},\cite{Palattella2016},\cite{Spiridon} discuss several aspects related to the evolution of these scenarios, their challenges, possibilities and limitations. This set of technologies or ecosystem has enabled the development of concepts such as Internet of Things, Smart Cities or Smart grids. Some of them, such as Bluetooth, 3GPP GSM,802.11g, NFC, have been massified by their use in devices such as mobile phones, computers, access control systems, sound systems, payment cards, etc., while others such as ZigBee, Lora,802.11p, are regarded as emerging technologies. In this context, with the rapid development of the wireless ecosystem, enormous challenges arise, such as opportunistic use of spectrum, regulatory matters, interoperability between technologies, quality of service and a key element: system security \cite{Frustaci2018}.

%\subsection {IoT ECOSYSTEM WIRELESS' TECHNOLOGIES}
%By classifying wireless technologies by range, we can talk about technologies: of proximity, WPAN, WFAN, WLAN, WNA and WWAN \cite{KeysightTechnologies2016}. 

%\subsubsection{PROXIMITY}
%Technologies such as NFC and EMVC are part of this group, which operate in a proximity range of up to 10 cm.

%\subsubsection*{NFC (\textit{Near-Field Communication})}   this is a short-range wireless technology \cite{Forum}, , based on the ISO 14443 standard that operates in the 13.56 MHz frequency band. It is used in access control systems, payments and varied types of transactions involving mobile phones \cite{Forum}.

%\subsubsection*{EMVC} \textit{Europay MasterCard VISA} is a standard that establishes the details of physical authentication between card integrated circuits and reading devices \cite{EMVCo}. It uses the communication protocol established in the standard ISO 7816-3, which defines commands for reading records, obtaining data, generating cryptograms, blocking and unlocking applications, among others.

%\subsubsection{WHAN:WIRELESS HOME AREA NETWORK}
%It brings together wireless technologies such as ZigBee, Z-Wave, Thread and Enocean, designed for interconnectivity of home devices, industrial control or home automation. They employ low data rates, ranging from 20 to 250 Kbps, and are generally designed to optimize power consumption.

%\subsubsection*{Zigbee:}a technology based on the IEEE 802.15.4 specification  \cite{Alliance}, , capable of operating in 2.4 GHz, 902MHz and 868 MHz bands, with transfer rates at 250 Kbps, 40 Kbps and 20 Kbps, respectively. It allows establishing star, tree, and mesh topologies.

%\subsubsection*{Z-Wave:}
%It is a short-range, low-power technology \cite{ITU2015}. Funciona en rangos de frecuencia por debajo de 1GHz: 868 MHz, 915 MHz y 920 MHz.  It works in frequency ranges below 1GHz: 868 MHz, 915 MHz and 920 MHz. Each network supports 232 devices. It is geared towards developing solutions such as remotely controlled lights, temperature sensors, remote door opening. The technical specifications are set out in the ITU G9959 standard.
 
%\subsubsection*{Thread:} Also based on the IEEE 802.15.4 specification for its physical and MAC layers \cite{ThreadGroup}; , and just like ZigBee allows to set up mesh topologies, but uses the standard (6LoWPAN) IPv6 on Low-power WPAN in its transport and network layers.

%\subsubsection*{6LoWPAN}
%An open standard defined by the IETF (Internet Engineering Task Force) in RFC 6282 \cite{Hui2011}, which specifies the structure of IPv6 datagrams for IEEE 802.15.4-based networks. The standard was designed for low-power networks. Regarding the 2.4 GHz band, it has been adapted for technologies such as Sub-1 GHz low-power RF, Bluetooth® Smart, power line control (PLC) and low-power Wi-Fi®. 

%\subsubsection*{Enocean}
%Technology developed by the German company EnOcean \cite{Enocean}. It was designed for the automation of buildings through the use of sensors that do not need batteries. Its products are powered using generator parts, photoelectric cells or thermocouples. It operates under the proprietary EnOcean wireless standard (ISO/ IEC 14543-3-1X) at frequencies 868 MHz for Europe and China, 902 MHz for North America and 928 MHz for Japan.

%\subsubsection{WPAN:WIRELESS PERSONAL AREA NETWORK}
%In this category fall technologies such as Bluetooth Low Energy, ANT+, MiWi and 802.15.4m, designed for the interconnection of devices used in environments close to people.

%\subsubsection*{Bluetooth Low Energy}
%Also known as Bluetooth Smart  \cite{BluetoothSIGInc}. Like Bluetooth, it operates on the 2.4 GHz ISM band (2.400—2.4835 GHz). Unlike Bluetooth, which has 79 channels with 1 MHz bandwidth, Bluetooth Low Energy was designed with 40 channels of 2 MHz bandwidth. It was created to consume less energy, optimizing technical parameters such as peak-current consumption.

%\subsubsection*{ANT+}
%ANT+ \cite{ANT+} is an Ultra Low-Power technology developed since 2012 by Dynastream \cite{DYNASTREAM}; which operates on the 2.4 GHz band with 125 channels and employs 8-byte messages. Among the leading manufacturers of these devices are Nordic Semiconductor \cite{NORDIC} and Texas Instruments \cite{TexasIntruments}.The technology is used in several sports and medical devices, and is compatible with Android mobile devices \cite{ANT+a}. 

%\subsubsection*{MiWi}
%MiWi \cite{Yang2010} is a technology based on the IEEE 802.15.4 specification, developed by Microchip Technology, available in some of its microcontrollers. It works in sub-GHz and 2.4 GHz bands.

%\subsubsection*{IEEE 802.15.4m}
%The IEEE 802.15.4m standard \cite{Sum} allows the use of digital television blanks for the operation of LR-WPAN, Low Rate-Wireless Personal Area Networks, at frequencies from 54 MHz to 698 MHz.

%\subsubsection*{IEEE 802.15.4p}
%Known as Positive Train Control \cite{IEEEStandard}. Technology developed for the monitoring and controling of the movement of trains. Works in the 220 MHz band.

%\subsubsection{WFAN:WIRELESS FIELD AREA NETWORK}
%This group includes wireless technologies for industrial applications such as ISA 100.11a, Wireless Hart and Wi-sun.


%\subsubsection*{ISA 100.11a}
%ISA 100.11a is a technology developed by the International Society of Automation \cite{ISA-100WirelessComplianceInstitute} with the ANSI/ISA-100.11a-2011 \textit{Wireless systems for industrial automation} standard, adopted by companies such as Honewell and Yokogawa. Its physical layer is based on the IEEE 802.15.4 standard. Its network and transport layers are TCP or UDP based with IPv6.

%\subsubsection*{Wireless Hart}
%Wireless Hart is based on HART, Highway Addressable Remote Transducer Protocol. It works in the 2.4 GHz band under IEC 62591 standard  \cite{Guidelines2016} and is part of 802.15.4 technologies.

%\subsubsection*{Wi-SUN}
%The physical layer of this technology \cite{Harada2017}, operates under the IEEE 802.15.4g standard, while the MAC layer does so pursuant to the specifications of the IEEE 802.15.4E standard. It is oriented towards the implementation of wireless networks for smart meters or M2M networks. It was adopted by Japan in power distribution companies. Products are grouped under the Wi-Sun Alliance \cite{Wi-SUNAlliance}.

%\subsubsection{WLAN: WIRELESS LOCAL AREA NETWORK}
%En esta categoría se agrupan las tecnologías 802.11 a/b/g/n This category groups widely used 802.11 a/b/g/n technologies; 802.11ac operates in the 6 GHz band with rates up to 6.9 Gbps, and 802.11ad can reach 7 Gbps in the 60 GHz band. Emerging technologies for this group include 802.11ah and 802.11p. The first is known as HaLow \cite{Wi-FiAlliance} and is aimed at low-power IoT applications with a range of up to 1 Km at frequencies below 1 GHz. The second is known as WAVE, wireless access in vehicular environments \cite{Jiang2008}, created for vehicle communications. 802.11af \cite{Flores2013} is known as super Wi-Fi or White-Fi  \cite{Holland2015} and allows the operation of local area networks in the blanks of digital television, in frequency bands between 54 and 790 MHz.

%\subsubsection{WNAN:WIRELESS NEIGHBORHOOD AREA NETWORK}
%Zigbee-nan and Wireless M-Bus technology fall within this classification.

%\subsubsection*{ZigBee-NAN}
%Its physical layer is based on the IEEE 802.15.4g standard and the MAC layer on IEEE 802.15.4e \cite{ZigbeeAlliance}.It is oriented towards the development of Smart Grids on a large scale. It works in ISM Sub-1 Gigahertz and 2.4 GHz, and uses network protocols such as IPv6,6LowPan (IPv6 over Low-Power Wireless Personal Area Networks \cite{Holland2015},  UDP, TCP, RPL (IPv6 Routing Protocol for Low-Power and Lossy Networks) [49] and CoAP (Constrained Application Protocol \cite{InternetEngineeringTaskForceIETF} y CoAP (\textit{Constrained Application Protocol} \cite{InternetEngineeringTaskForceIETF2014},\cite{CoAP}, , with multicast capabilities for the implementation of M2M communications in mesh topologies.

%\subsubsection*{Wireless M-Bus}
%Denomination for the European standard EN 13757-4 used for remote reading of energy and gas meters \cite{M-Bus} \cite{Mohan2015}.The wired variant is the M-Bus. Its operating frequencies are 169 MHz,433 MHz and 868 MHz.
 

%\subsubsection{LPWA:LOW POWER WIDE AREA - SIN LICENCIA}
%The LORa, SIGFOX, Telensa technologies that can be considered emerging are grouped in the category of unlicensed LPWA \cite{Mekki2018}.Other members of this group include OnRamp and Positive Train Control. LPWAN technologies seek to develop devices that send little data over a wide area, with a battery span of several years.

%\subsubsection*{LoRa}
%LoRa (\textit{Long Range}) \cite{Alliancea} is a technology that enables two-way communications using free-use frequency bands: 433 MHz, 470 MHz, 868 MHz and 915 MHz. Among its advantages is the long range (approximately 10 km) of communication between the devices and the gateway, as well as its low power consumption \cite{Semtech}. Its physical layer uses a modulation technique known as Chirp Spread Spectrum (CSS). LoRaWAN is an open standard where communications protocol and media access control (MAC) are set in the data-linking layer.

%\subsubsection*{SIGFOX}
%a proprietary technology of the French company Sigfox \cite{SigFox}.this company operates as a global communications operator for its technology. It has coverage in 50 countries, grouped into six geographical areas that define the operating frequency bands of wireless devices ranging from 862 to 928 MHz. Its topology is a star where nodes send short messages to a SigFox base station (gateway). The base station modulates messages and sends them to the Sigfox cloud. A SigFox cell can cover a range of 20-50 km in rural areas and between 3 and 10 km in urban areas.

%\subsubsection*{Telensa}
%Developed by the English company Telensa \cite{Telensa}, , and based on Ultra Narrow Band (UNB) radio technology, it employs ISM Sub-1 GHz bands. A base station can connect 5000 nodes with a coverage of 2Km in urban areas and 4Km in rural areas. It has large-scale applications for lighting control in large cities, especially from the United Kingdom.

%\subsubsection*{On-Ramp Wireless}
%Also known as INGENU \cite{INGENU}. This is a technology developed for M2M solutions that allows linking up to 48 Km in the 2.4 GHz free-use band. Based on proprietary Random Phase Multiple Access technology. 

%\subsubsection{LPWA:LOW POWER WIDE AREA - CON LICENCIA}
%The other category of LPWA corresponds to licensed technologies, where 3GPP NB-IoT appears. This technology allows the development of LTE hardware with specific features for IoT solutions.

%\subsubsection*{NB-IoT}
%\textit{Narrowband Internet of Things} \cite{Finnegan2018} is based on LTE technology, with modifications defined in 3GPP revision 13. Works on licensed frequency bands. NB-IoT uses a reduced bandwidth of 180 kHz compared to the 1.4-20MHz used by LTE. It seeks to be able to manage 52000 devices per channel, per cell.

%\subsubsection*{EC-GSM-IoT}
%This is another technology for IoT development defined by 3GPP  \cite{Finnegan2018}. It uses bandwidth of 200 kHz per channel, with a total bandwidth of 2.4 MHz, and proposes the use of existing GSM infrastructure and support 50000 devices per cell, with transmission rates between 350 bps at 70 Kbps.





==> A Technical Review of Wireless security for the Internet of things_/3_sdr.tex <==
%\subsection{DEFINITION}
In 2009, the ITU-R International Telecommunication Union Working Group 1B defined the term SDR (Software-Defined Radio) for the 2012 World Radio communication Conference \cite{ITU-R2009}, as: “A radio transmitter and/or receiver employing a technology that allows the RF operating parameters including, but not limited to, frequency range, modulation type, or output power to be set or altered by software, excluding changes to operating parameters that occur during the normal pre-installed and predetermined operation of a radio according to a system specification or standard.” Already in 1992, Joseph Mitola III \cite{MitolaJ1999} had defined the term software Radio as: “A software Radio is a radio wave channel modulations waveforms are defined in software.That is, waveforms are generated as sampled digital signals, converted from digital to analog via wideband DAC (Digital Analog Converter) and the possibly unconverted form IF (Intermediate Frequency) to RF (Radio Frequency) .The receiver, similar, employs a wideband ADC (Analog to Digital Converter) that captures all the channels of the radio node software. The receiver then extracts, down converts and demodulated the channel waveform using software on a general purpose processor.”

%\subsection{SDR ARCHITECTURES}

%In his definition \cite{Mitola2000},  Mitola describes the main elements that make up a software-defined radio. The transmission of the radio frequency signal requires a broadband digital analog converter (DAC) coupled with an up-conversion process from an intermediate frequency to radio frequency. The reception needs a digital analog converter, also broadbanded, and a down-conversion process followed by a process of demodulation of signals, using algorithms implemented in some type of processor. This definition has been implemented over the years by developing some architectures implemented in hardware. In the evolution towards an ideal SDR radio system, it has been sought to move the analog digital and digital analog conversion processes as close as possible to the antenna, so that all signal processing can be done digitally. 
%\begin{figure}[h]
%        \centering
%        \caption{Ideal SDR radio. Based on \cite{Mitola2001}, Fig 9.}
%        \includegraphics[width=0.45\textwidth]{images/Mitola.pdf}
%       \label{fig:radiomitola}
%\end{figure}

%The SDR hardware design has been framed in the evolution of microelectronics and its ability to improve the performance of ADC and DAC converters; however, the designers of integrated circuits of radio frequency try to solve problems arising from the direct relationship between power consumption and sampling rate in the converters. In 1999, Mitola  \cite{Mitola1999} presented in a SDR classification scenario, radio systems for some types of hardware. Figure \ref{fig:radiomitola} shows the ideal SDR radio at point (X), located at the point of convergence where the bandwidth for ADC and DAC converters are in the order of the GHz and we can speak of Digital Radio Frequency, operating under a general-purpose hardware architecture. In the graph are located radios such as STR 2000 (Point A), based on DSPs architectures, with bandwidth around kHz. Point (B) shows the Cost Handset radio developed using application-specific integrated circuits (ASIC) technology in a frequency range also around kHz. For point (C), radio SWR Cell site, the bandwidth frequency for ADCs and DAC increases around MHz. For the case (D), Radio Speak Easy II, the frequency is kept around MHZ, but using DSP technologies in the construction thereof. MIT's Virtual Radio, located at point (V) of the figure, is classified as general-purpose design technology for bandwidth frequencies around MHz.

%At present, three major types of architectures for SDR systems can be discussed: direct sampling, super-heterodyne and direct conversion radio \cite{Holland2015}. SDR architectures oriented to the design of cognitive radio solutions are discussed in \cite{Arslan2007}.

%\subsubsection{Direct Sampling Radios}
%The direct sampling architecture, in Figure \ref{fig:SDR_ideal}, is ideal for a software-defined radio transmission and reception system. Its purpose in reception is the digitization of the radio frequency signal coming from the antenna, and achieves it by means of a digital analog converter (ADC) \cite{Holland2015}.It uses an analog Digital converter (DAC) in its operation as a transmitter, the output of which is amplified and sent via an antenna. This type of architecture is successfully used in specialized areas such as radio astronomy, where receivers are located in areas with very little interference. Its big drawback has to do with the power consumption by converters, which makes this system impossible for mobile devices.

%\begin{figure}[!th]
%        \centering
%        \caption{Direct sampling SDR architecture. Based on \cite{Holland2015}, Fig 1.1}
%        \includegraphics[width=0.45\textwidth]{images/SDR_modelo_1.pdf}
%       \label{fig:SDR_ideal}
%\end{figure}

%\subsubsection{Superheterodyne}
%A superheterodyne system uses an intermediate frequency to facilitate the digitization of signals in a band where the converter can operate optimally. Receivers manufactured with this type of architecture are used in high-performance applications for very-narrow-frequency ranges. Their level of integration is low.

%\subsubsection{Direct Conversion Radios}
%This architecture has become the most widely used to design both SDR hardware and digital radio systems in general. In a receiver designed under this architecture, the radio frequency signal is amplified and passed through a band-pass filter before converting it to a baseband signal in quadrature or complex representation. Most analog channel filtering is done in baseband, where these processes can be easily integrated into semiconductors. The advantage of this type of architecture is its simplicity, especially when used in applications with high bandwidth, and that each ADC converter operates at half the sampling rate. Their disadvantage is that they require dual converters, as well as two paths for baseband I and Q signals, which may turn out not to be exactly symmetrical, and may cause differences in quadrature gain or phase imbalance caused by some mixers or signal processing in baseband. Furthermore, because the baseband process drops down to 0 Hz, small DC offsets in this process can cause foamy signals centered on the band of interest. Due to the popularity of direct conversion receivers, several OFDM-based standards such as LTE or 802.11 a/g/n/ac currently avoid using the central part of the band for this reason. 

%\subsection{STRUCTURE OF AN SDR SYSTEM}
%Figure \ref{fig:sistema_com_dig} shows the model of a digital communication system, where the subsystems that make up both the transmitter and the receiver are identified. Processes can occur at the level of bits, symbols or analog signals. The process starts at the transmitter, with the source of the data. Once there, analog signals coming from the real world, such as voice or images, are converted into digital signals with binary representation through sampling and quantization processes. This binary information passes into a source encoding block, which seeks to generate as short as possible and equally likely bit strings. This process uses encodings such as Hufman, Lempel-Ziv, Fano, etc. The output data enters subsequent stage where the channel encoding occurs, which introduces controlled redundancy in order to detect or correct errors in the receiver. This process can use different types of codes such as linear blocks, convolutional blocks, cyclic redundancy, LDPC, etc. 
 
% \begin{figure}[h]
%        \centering
%        \caption{Digital communication process}
%        \includegraphics[width=0.48\textwidth]{images/system_COM_dig.pdf}
%        \label{fig:sistema_com_dig}
%\end{figure}

%The digital data obtained then moves on to the processes of converting bits to symbols and the modulation process is performed, which modifies the amplitude, frequency or phase parameters of a carrier signal depending on the type of digital modulation. In an SDR system, digital signals are converted to analog by a digital-to-analog converter (DAC) device. The analog process occurs in a radio frequency interface that moves the baseband signal to an RF frequency. This signal is carried to the medium by means of an antenna. In the channel, the signal is affected by variations in radio propagation phenomena and by various types of noise.
%Subsequently, the receiving device, by means of an antenna, captures the signal from the medium and takes it to a radio frequency interface, where it moves to the baseband frequency. The received analog signal is then converted into a digital signal using an analog digital converter (ADC). The rest of the process occurs digitally. The data obtained from the converter are demodulated, and then proceed to the decoding of the channel, where an error check is performed, and depending on the error control technique implemented in the transmission, the algorithm in the receiver can detect the errors or even correct them. Once the bit sequence appears in the output of the channel decoder of the receiver, the decoding of the source occurs, which finally delivers the received data to the receiving end. 

%This whole process corresponds to the digital communication system model proposed by Claude Shannon in 1948 \cite{ClaudeE.Shannon1948}. Regardless of the type of technology or its operating frequencies, the designs of transmitters and receivers specified in the technical standards for each of the wireless technologies that make up the ecosystem of the Internet of Things follow these processes. When assessing the vulnerabilities of a wireless communication technology, any of the subsystems or blocks that make up the digital communication system may be susceptible to modification or pose some kind of risk.

%\subsection{I-Q SIGNAL REPRESENTATION}
%By processing I/Q signals, it is possible to implement any type of modulation or digital demodulation. There is a correlation between analytical representation and hardware implementation of direct-conversion radio architectures.For analytical development, representation by complex exponentials facilitates mathematical development.Figure \ref{fig:IQ_1} shows the vector representation of an I/Q signal. The vector of magnitude $A(t)$ with angle  $\varphi$ can be represented in a variety of ways.      
%\begin{figure}[h]
%        \centering
%        \caption{I-Q representation of the X(t) signal }
%        \includegraphics[width=0.35\textwidth]{images/I_Q.pdf}
%        \label{fig:IQ_1}
%\end{figure}
%In quadrature processing, the actual part is called the phase component and the imaginary part is called the quadrature component.The  $Y(t)$ signal can be defined as:

%\begin{equation}
%\label{eqn:uno}
%Y(t)=A(t)\cos(\omega_ot+\varphi(t))\\
%\end{equation}
%Applying trigonometric identities, the
% \ref{eqn:uno} can express as:
%\begin{equation}
%\label{eqn:dos}
%    Y(t)=A(t)\cos(\omega_ot)\cos(\varphi(t)-A(t)\sin(\omega_ot)\sin(\varphi(t))\\
%\end{equation}
%where:
%\begin{equation} \label{eq1}
%\begin{split}
%i(t)=A(t)\cos(\varphi(t)) \\
%q(t)=A(t)\sin(\varphi(t))
%\end{split}
%\end{equation}
%So that:
%\begin{equation}
%Y(t)=i(t)\cos(\omega_ot)-q(t)\sin(\omega_ot)
%\end{equation}

%For a transmitting system, the $Y(t)$ signal can be obtained by the system shown in Figure 6. \ref{fig:TX_IQ}. The signal  $i(t)$ multiplied by $cos(\omega_ot)$ is known as the signal in phase I and the signal $q(t)$ multiplied by $-sin(\omega_ot)$ corresponde a la señal en cuadratura Q.corresponds to the signal in quadrature Q. The sum of these two signals is known as the modulated signal.

%\begin{figure}[h]
%        \centering
%        \caption{I/Q Transmission System}
%        \includegraphics[width=0.45\textwidth]{images/phase_quadrature.pdf}
%        \label{fig:TX_IQ}
%\end{figure}

%Figure \ref{fig:sistemaIQrx}represents the receiving process. Using this design, the I/Q components are obtained independently.The received $Y(t)$ signal is multiplied by two signals: a $cos(\omega_ot)$ signal in channel I and a $-sin(\omega_ot)$ signal in channel Q. The phase and quadrature components $z_1(t)$ and $z_2(t)$ are obtained after applying a low-pass filter on each of the channels.

%\begin{figure}[h]
%        \centering
%        \caption{I/Q receiving system}
%        \includegraphics[width=0.45\textwidth]{images/RX_model.pdf}
%        \label{fig:sistemaIQrx}
%\end{figure}

%The design of digital transmission and reception systems requires implementing digital signal processing stages such as digital signal filtering and carrier synchronization techniques. Moreover, in order to limit the bandwidth of transmissions and avoid inter-symbol interference, during the process of converting bits to symbols, it is necessary to implement processes known as pulse shaping that use RC (Raised Cosine) or RRC (Root Raised Cosine) filters.In  \cite{Collins2018},\cite{Grayver2013},\cite{Atkinson} are discussed the elements necessary for the design of digital communications systems based on SDR architectures.

\subsection{SDR Hardware Platforms}

The concept of SDR platforms arose with Mitola in 1992 \cite{Mitola1993}.In 1996, at MIT, the \textit{SpectrumWare software radio project} was carried out, where a prototype receiver of a GSM base station was developed \cite{Tennenhouse1996}.In 1999, SDR SpeakEasy I/II radios were manufactured, for military use, and financed by the US government.In 2004,  the company Ettus was created and the production of SDR-USRP hardware began; its use has expanded and has become one of the most widely used platforms nowadays \cite{Machado2015},\cite{Pawelczak2011},\cite{Mitola2015}. 

Table \ref{tab:ADC-DAC} presents a summary of the technical characteristics of some commercially available software-defined radio platforms: The number of bits used by analog digital and/or digital analog converters is regarded (DAC), as well as their sampling rates, bandwidth and transmission, and/or reception possibilities.

The increase in the sampling capabilities of converters attests to the evolution of SDR platforms, which enables the implementation of modern wireless communications standards \cite{Machado2015}. SpeakEasy used converter devices with sampling rates in the order of 200 Kb/s for its manufacture in 1999 \cite{Cook1999}.The USRP1, designed in 2004, has an ADC converter sampling rate of 64 [MS/S], compared with the reference USRP X310 released to the market in 2016; the sampling rate is observed to have increased to 200 [MS/s]. The evolution of the platforms has also allowed the increase of radios' frequency range. As can be seen in the  table \ref{tab:ADC-DAC} the frequency ranges reach 6 GHz.
  \begin{table}[h!]
%      \centering
   % \begin{tabular} { m{5em} c{3em} m{6em} m{2em} m{2em} } 
   \begin{tabular} { m{10em} p{3em} m{3em} m{3em} m{4em} }
    
 %   \begin{tabular}{lllccc}
        \hline
      \textbf{Platform} & \textbf{ADC /DAC [Bits]} & \textbf{ADC /DAC [MS/s]} & \textbf{Tx/Rx} & \textbf{Fmin-Fmax [MHz]}\\
%      \begin{tabular}{*{10}{l}}
        \hline
%       \textbf{Año} & \textbf{Plataforma} & Bits &Muestreo ADC  \\
     %   SpeakEasy \cite{Cook1999} & - & 200 Kb/s & - & -  \\
     %   \hline
        RTL \cite{RTL-SDR.COM} & 8/- & 3.2/- & Rx & 25-1750  \\
        \hline
        FUNCube \cite{FUNcube} &  16/- & 96 KHz  & Rx & 64-1700  \\
        \hline
        Airspy-mini \cite{Airspy} & 12/- & 20/- & Rx & 24-1700  \\
        \hline
        HackRF One \cite{HackRFOne} &  8/10 & 20/20 & Tx-Rx & 1-6000  \\
        \hline
        Pluto \cite{AnalogDevices} &  12/12 & 61.4 /61.4 & Tx-Rx & 325-3800 \\
        \hline
        BladeRF 2.0 Micro \cite{Nuand} & 12/12 & 61.4 /61.4 & Tx-Rx & 47-6000  \\
        \hline
        USRP-1 \cite{EttusResearchc}& 12/14 & 64/128 & Tx-Rx & DC-6000  \\
        \hline
        Nutaq PicoSDR \cite{Nutaq}&  12/12 & 80/80 & Tx-Rx & 56-6000  \\
        \hline
        USRP-2 \cite{EttusResearchc}& 14/16 & 100/400 & Tx-Rx  & DC-6000  \\
        \hline
        USRP-N210 \cite{EttusResearchc}& 14/16 & 100/400 & Tx-Rx  & DC-6000  \\
        \hline
         WARP-V3 \cite{MangoCommunications} &  12/12 & 100/170 & Tx-Rx & 2400/5000  \\
        \hline
        LimeRF LMS7002M \cite{LimeMicrosystems} &  12/12 & 160/640 & Tx-Rx & 0.1-3800  \\
        \hline
        USRP X310 \cite{EttusResearchc}&  14/16 & 200/800 & Tx-Rx & DC-6000  \\
        \hline
      % USRP serieX \cite{EttusResearchc}&  14 & 200 & 16 & 800  \\
      % \hline
       % BladeRF x40 \cite{Nuand} &  12 & 40 & - & -  \\
       % \hline
        USRP N310 \cite{EttusResearchc} &  16/14 & 153.6 /153.6 & Tx-Rx & 10-6000  \\
        \hline
        AIR-T \cite{Digital} &  12/10 & 245.7 /245.7 & Tx-Rx & 300-6000  \\
        \hline
        CRIMSON \cite{Pervices} &  16/16 & 370,16 /2500,16 & Tx-Rx & 0.1-6000  \\
        \hline     
      %  YARD-Stick \cite{GreatScottGadgets} &  - & - & - & 300-348  391-464   782-928   \\
      %  \hline
      \end{tabular}
      \\
      \caption{\label{tab:ADC-DAC} Software Defined radio platforms comparison}

    \end{table}




In addition to improvements in the features of radio interfaces, SDR hardware has also evolved in increasing its computational capacity by integrating DSP and FPGAs devices into its systems.The \textit{Xilinx Virtex 6} is used in SDR devices such as PicoSDR, WARP v3; the X-Series USRP uses \textit{Xilinx Kintex 7} FPGAs and platforms such as CRIMSON \cite{Pervices} integrate an \textit{FPGA-Arria V ST SOC} and an \text{ARM Cortex-A9 MP}. The AIR-T(\textit{Artificial Intelligence Radio - Transceiver }) platform \cite{Digital} combines a 2x2 SDR MIMO system with a 256-core  \textit{GPU Jetson TX2} on a single card.Its ADC and DAC converters reach sample rates of up to 245.7 [MS/s]. Other platforms can be classified in the low-cost hardware category such as RTL \cite{RTL-SDR.COM}, HackRF  \cite{HackRFOne},AirSpy \cite{Airspy},FUNCube \cite{FUNcube},BladeRF \cite{Nuand}, LimeRF \cite{LimeMicrosystems} and Pluto \cite{AnalogDevices}; These devices, along with free software tools such as GNU Radio and driver integration for SDR devices signal processing platforms such as Matlab and Labview have enabled the development of software-defined radio technology worldwide.

 
%\subsection{UNIVERSAL RADIO SOFTWARE PERIPHERAL-USRP}

%Figure \ref{fig:sistemaIQ} shows the USRP radio architecture model \cite{EttusResearch}. The system consists of a radio frequency card (daughterboard) and a digital signal processing system based on an FPGA. The daughterboard contains the analog elements that make up the radio frequency transmission and reception stages. The transmission and/or reception is selected via an RF switch. The receiving process, amplifies and filters the signal from the antenna before reaching the ADC converter. Similarly in the transmission stage that occurs on the daughterboard, I/Q signals from the DAC are filtered and multiplied by the mixers with the reference signals, and then amplified. 

%System synchronization is achieved through an external signal or through a synchronisation phase based on PLL devices. Digital processes such as decimation, interpolation, downconversion and upconversion occur in FPGA, where radio transport protocols are implemented, which allow controlling both transmission and reception. I/Q signals are sent or received to or from a computer via communication interface, which depending on the reference of the USRP device can be USB 2.0, 3.0, Ethernet: Gigabit or 10 Gigabit or PCI Express. I/Q signals that are sent or received are organized in formats such as \textit{Little Endian} or \textit{Big Endian}. Figure \ref{fig:sistemaIQ}  shows the case of 16-bit I/Q packets each and how they are structured according to format. USRP platforms use the \textit{Big Endian} format where a package contains 16 bits I followed by 16 bits Q, organized into a 32-bit word.

%\begin{figure*}[t]
%        \centering
%        \caption{USRP platform. Based on \cite{EttusResearch}. }
%        \includegraphics[width=1\textwidth]{images/USRP_board.pdf}
%        \label{fig:sistemaIQ}
%\end{figure*}

%\subsubsection{DAUGHTERBOARD - USRP}
 
%Table \ref{tab:Tarjetas_hijas} shows the various RF card references for USRP platforms and their equivalence with National Instruments radio platforms \cite{NationalInstruments},\cite{EttusResearchc}.Each of the cards has a frequency range and a bandwidth. Cards with the same frequency range can have different bandwidth. The most modern references can reach bandwidth up to 160 MHz.

%\subsubsection{USRP}
%   \begin{table}[h]
%      \centering
%      \begin{tabular}{*{2}{lllc}}
%      \begin{tabular}{*{10}{lllc}}
%        \hline
%       \textbf{Ettus} & \textbf{NI} & \textbf{Frequency (MHz)}& \textbf{BW (MHz)}\\
%        \hline
%       LFRX/LRTX & - & DC-30  & 30  \\
%        \hline
%       WBX & 2920 & 50-2200 & 40  \\
%        \hline
%       WBX-120 & 2940 & 50-2200 & 120  \\
%          \hline
%       WBX-160 & - & 50-2200 & 160  \\
%          \hline
%       SBX & 2922 & 400-4400 & 40  \\
%        \hline
%       SBX-120 & 2942 & 400-4400 & 120  \\
%        \hline
%       SBX-160 & - & 400-4400 & 160  \\
%        \hline
%        XCVR-2450 *& 2921  & 2400-2500/4900-5900 & 40  \\
%        \hline
%        CBX & 2943 & 1200-6000 & 40  \\
%        \hline
%        CBX-120 & 2943 & 1200-6000 & 120  \\
%        \hline
%         CBX-160 & - & 1200-6000 & 160  \\
%        \hline
%        UBX & - & 10-6000 & 40  \\
%        \hline
%        UBX-160 & 2944 & 10-6000 & 160  \\
%        \hline
%      \end{tabular}
%      \caption{\label{tab:Tarjetas_hijas} Ettus daughterboard - NI. \cite{EttusResearch} }
%     
%    \end{table}

%\subsubsection{RADIO PACKET PROTOCOLS}
%Packet protocols are used for the exchange of samples or control parameters between radio and external communication interfaces. VRT (VITA Radio Transport protocol) has been used for USRP devices. Third generation devices and the B200, use a specific protocol of the company Ettus, the CHDR (compressed header).

%\subsubsection*{VRT}
%\textit{VITA Radio Transport protocol} \cite{Grayver2013}  is an open radio protocol defined by the VITA-49 standard  \cite{VITA}.It enables interoperability between different types of radios and software systems. For USRP devices that work with the UHD driver, only a portion of the standard was implemented.

%\subsubsection*{CHDR}
%CHDR (\textit{compressed header}) \cite{EttusResearch}  is a radio transport protocol developed by Ettus for its third generation radios. It uses a fixed-length 64-bit header, which is managed in the FPGA along with the AXI streaming protocol. Ettus has arranged a library for the analysis of the protocol using Wireshark in \cite{EttusResearcha}. 


%\subsubsection{COMMUNICATION INTERFACES}
%Table \ref{tab:interfaces_USRP}  describes the types of communication interfaces for SDR-USRP platforms. Considering the transmission and reception of 16-bit I/Q signals, the lowest transfer rate corresponds to the USB 2.0 interface, included in USRP1 and B100 platforms, with 8 MS/S. The highest rate can be reached with the PCI-Express interface where it can reach 200 MS/s. On most USRP platforms, the sample size can be set to 8 bits, thus doubling the transfer rate of the communication interface. The Half-Duplex or Full-Duplex mode refers to the possibility of having simultaneous communication through the communication interface. Only USB 2.0 and USB 3.0 ports have Half-Duplex mode, the other platforms can reach the transfer rates indicated in the table with simultaneous transmission and reception communication via the communication interface.


%  \begin{table}[h]
%      \centering
%      \begin{tabular}{*{10}{llc}}
%    \begin{tabular} { m{5em} m{7em} m{3em} m{6em} } 
%        \hline
%       \textbf{Interface} & \textbf{Plataform} & \textbf {Rate (MS/s)  16-bit I/Q} & \textbf{Mode} \\
%        \hline
%        USB 2.0 & USRP1/B100 & 8 & Half Duplex \\
%        \hline
%        Gigabit Ethernet & N200/N210 & 25 & Full Duplex \\
%        \hline
%         Gigabit Ethernet & N200/N210 & 25 & Full Duplex\\
%        \hline
%        PCI-Express (1-lane PCIe Card) & X300/X310 & 50 & Full Duplex \\
%        \hline
%         USB 3.0 & B200 B210 B200mini B205mini & 61.44 & Half Duplex\\
%        \hline
%        PCI-Express (4-lane PCIe Card) & X300/X310 & 200 & Full Duplex\\
%        \hline
%      \end{tabular}
%      \caption{\label{tab:interfaces_USRP}Communication interfaces for USRP platforms. \cite{EttusResearch}}
%     % \caption{Tasas de muestreo para diversas plataformas }
%    \end{table}

%\subsection{SOFTWARE FOR SDR}

%Software-defined radio technology hardware platforms require communication drivers and software to enable the processing of sampled radio signals. Among the most used software are: GNU Radio \cite{GNURADIO}, Matlab \cite{Mathworks}, Labview \cite{NationalInstruments},Redhawk \cite{Redhawk} and OSSI \cite{OSSIE}.The most well-known driver is the UHD, developed by the company Ettus for communication with its USRP hardware platforms.

%\subsubsection{UHD }
%The USRP Hardware Driver \cite{EttusResearchb} enables USPR devices to communicate with several software platforms. It provides the necessary information to transport signals to and from the USRP hardware along with the control parameters. It is available under the GNU Open Source License (GPLv3). It was written in C/C++ language.

%\subsubsection{GNU RADIO}
%Project created by Eric Blossom in 2001 \cite{GNURADIO}. In 2009, Josh Blum developed the graphical interface GNU Radio Companion, a tool that contains the elements necessary to create multiple architectures for the processing of radio signals. Through the interconnection of the set of blocks, programmed in C++, and communication with hardware platforms, it allows to implement various radio communication systems.


%\subsubsection{MATLAB}
%Mathworks included in its Matlab and simulink libraries functions and blocks that allow working directly with software-defined radio hardware such as: USRPs, RTL, ADALM-PLUTO and Analog Devices evaluation cards such as PicoZed SDR or ZedBoard,\cite{Mathworks}.In \cite{Atkinson} y \cite{WyglinskiAlexanderM.2013}, Matlab is used together with USRP hardware, as a tool for the learning concepts in a communication systems course.

%\subsubsection{LABVIEW} 
%National Instruments \cite{NationalInstruments},acquired Ettus in 2010, and since then the SDR hardware for NI has equivalencies to radios manufactured by Ettus as can be seen in the Table (\ref{tab:Tarjetas_hijas}).The Labview software uses the UHD driver to establish communication between its blocks and the SDR hardware.

%\subsubsection{REDHAWK}
%Redhawk \cite{Redhawk} is a free-use SDR working environment. Its graphic environment was developed by Eclipse. It is the evolution of the OSSIE tool \cite{OSSIE}.It is compatible with the SCA standard  (\textit{Software Communications Architecture}. 

%\subsection{REGULATORY ASPECTS}
%Standardization of SDR technology is a task that highlights two major initiatives: the JTRS/SCA standard developed by the United States Army and the STRS created by NASA.   Companies manufacturing commercial radios such as Ettus  \cite{EttusResearch} and Nutaq  \cite{Nutaq}, have developed or adapted some of the existing architectures to the design of their products.

%\subsubsection{JTRS/SCA}
%The use of radios with very diverse technical characteristics by the forces of the United States Army caused problems when coordinating operations, which led to the need to develop radios with SDR technology. In 1997, the Joint Tactical Radio System programme \textit{Joint Tactical Radio System} \cite{Way2013}, was created to facilitate software exchange between various SDR radio platforms. The main standard developed by the JTRS program was the SCA (Software Communications Architecture). Since 2015, the latest standardization revision was approved: SCA 4.1 (\textit{Software Communications Architecture}). 

%Standardization defines APIs (\textit{Application Programming Interfaces}) that allow interaction with radio platforms to facilitate portability and reuse of applications. The standard is used by manufacturers for the development of their products in civil and military applications.

%\subsubsection{STRS} 
%\textit{Space Telecommunications Radio System }(STRS) \cite{STRS} is a standard that defines an open architecture for the development of SDR radios used in space applications and earthly stations \cite{Kacpura2014},\cite{Kacpura2015}. This standardization seeks to define architectures that allow reusing services and signals implemented in SDR through different platforms in order not to depend on a single provider. SDR radio platforms operating under this architecture are: SPARC, developed by JPL (\textit{Jet Propulsion Laboratory}-NASA) \cite{NASA-JPL};Starlight and ColdFire designed by \textit{General Dynamic Corporation} \cite{GeneralDynamics}; SDR-3000 and Starlight developed by GRC  (\textit{Glenn Research Center}-NASA) \cite{Heidman2015} and AiTech designed by Harris  \cite{Harris}.


==> A Technical Review of Wireless security for the Internet of things_/4_ciberseguridad.tex <==
To assess the vulnerability level of a system or technology, the \textit {National Infrastructure Advisory Council (NIAC)} \cite{NIAC} established the \textit{Common Vulnerability Score System} (CVSS) \cite{CVSS}.  \cite{Qu2016} uses this classification to perform a vulnerability assessment on Bluetooth low energy technology in IoT systems. Moreover, the U.S. Department of Homeland Security, through the Office of Cybersecurity and Communications (CSC), set up a mechanism to identify and classify attack patterns through a public catalog known as CAPEC (\textit{Common Attack Pattern Enumeration and Classification})\cite{CAPEC}. 

%This section includes some important definitions and concepts related to cybersecurity, taking into account sources such as \cite{Moura2012},\cite{Heinaaro2015},\cite{Baldini2012},\cite{Frustaci2018},\cite{Al-SakibKhanPathan2016} and \cite{Maini2018} ; Next, there will be a classification of SDR radios vulnerabilities and a description of the wireless IoT ecosystem's most common wireless vulnerabilities. The types of attacks directed towards cognitive radio networks are also listed. Afterwards, experiences of implementing various types of wireless attacks using SDRs devices are detailed. Finally, some cases of using SDR platforms as a tool for cybersecurity analysis are reported.
 
%\subsection{DEFINITIONS}

%Taking into account \cite{Moura2012} important concepts such as Attack, intrusion and vulnerability are defined.

%\subsubsection{ATTACK}
%An attack can be defined as a malicious action that seeks to exploit one or more vulnerabilities in a communication system, which may affect its functioning. Attacks can be passive or active. In a passive attack, the attacker aims to obtain information or affect the system, but seeks not to be detected; this makes it more difficult to identify such attacks. In an active attack, the attacker seeks to exploit wireless protocol security deficiencies present in the various layers of the OSI model. The attacker, in these cases, may not mind going unnoticed. Attacks can also be classified as internal or external. An external attack originates outside the network and its damage can be limited to a small area, while an internal attack can have a very large impact on the operation of the entire system.

%\subsubsection{VULNERABILITY}
%This is a system defect that can affect its security; it may be associated with hardware or software. Vulnerabilities can be in design, implementation, or operational.

%\subsubsection*{Design Vulnerability:}UA design vulnerability occurs during system design and may be associated with the use of a weak encryption mechanism, the implementation of a protocol susceptible to some kind of attack, or selecting hardware that does not allow the implementation of security features. These design failures can be intentional or associated with factors such as lowering device implementation costs.

%\subsubsection*{Deployment Vulnerability:}It may occur in the manufacturing process of a product or in the supply chain. It can be both hardware and software- related. One of the vulnerabilities may be the introduction of some type of Trojan during the radio manufacturing process; another may be the cloning of the hardware during the manufacturing process.

%\subsubsection*{Operational vulnerability:}It may occur in the manufacturing process of a product or in the supply chain. It can be both hardware and software- related. One of the vulnerabilities may be the introduction of some type of Trojan during the radio manufacturing process; another may be the cloning of the hardware during the manufacturing process.

%\subsubsection{INTRUSION} 
%This is an attack that becomes successful by exploiting some vulnerability. An attack exploits a vulnerability and becomes an intrusion due to the existence of a breach in the security policy of the system.
\subsection{MOST COMMON WIRELESS VULNERABILITIES}

According to \cite{Fragkiadakis2013}, the security basics for the operation of a wireless network are confidentiality, integrity, availability and access control. Confidentiality must ensure that network data cannot be read by unauthorized users, while integrity detects intentional or accidental changes to data being carried over the network. Availability ensures that devices and users can use the network and its resources when they need it, and access control restricts resources to authorized users only. 

The company Bastille Networks conducted a classification of the top 10 vulnerabilities of wireless systems \cite{BastilleNetworks}.Table \ref{tab:bastille} describes each one. 

%Solutions for the diagnosis or control of these vulnerabilities are based on software-defined radio technologies.

\begin{table}[h!]
\small
    %\centering
    %\begin{tabular}{p{5cm} p{12cm}}
    \begin{tabular}{p{2cm}p{6cm}}
    \hline
    %\begin{tabular}{l l}
    \textbf{Vulnerability} & \textbf{Description}  \\
    \hline 
    \textit{Rogue cell towers} & It use IMSI catchers or Stingrays. A mobile cell allow spoof an cellular communication. The attacker can heard and read SMS.\\
  %  Celda móvil que permite al atacante intervenir una comunicación celular pudiendo escuchar llamadas y leer mensajes de texto.Emplean dispositivos IMSI catchers o stingrays
    \hline
    \textit{Rogue WiFi Hotspots} & The WiFi hotspots can be used to deploy man in the middle attacks. Is possible keep watch on network traffic or stole user's credentials.\\
%    Los puntos de acceso WiFi pueden usarse para ataques tipo \textit{Man in the Middle} mediante los cuales se puede espiar el tráfico de la red o robar credenciales de los usuarios\\
    \hline
    \textit{Bluetooth Data exfiltration} & It uses a mobile device with Bluetooth that avoids network controls by means of internet access across the cellular network.\\
%Un dispositivo móvil con bluetooth puede ser usado para dar acceso a internet a través de una red de telefonía móvil, evitando los controles de seguridad de la red. \\
    \hline
    \textit{Eavesdroping / surveillance devices} & Eavesdropping devices voice-activated, with FM or GSM transmission. Devices are hidden in offices or meeting rooms.\\
   % Dispositivos de escucha o vigilancia, activados por voz con transmisión en frecuencia modulada o GSM. Escondidos en oficinas o salas de conferencia.
    \hline
    \textit{Vulnerable wireless peripherals} & keystroke injection attacks. It uses the weakness of wireless keyboards and/or mouses without data encryption.\\
    
   % Teclados o \textit{mouses} inalámbricos pueden ser espiados o suplantado debido a que no tienen encripción de datos. Permiten un ataque conocido como \textit{keystroke injection}.\\
    \hline
    \textit{Unapproved cellular device presence} & Unapproved cellular device use in restricted areas. \\
    %Uso no autorizado de dispositivos celulares en áreas especificas.
    \hline
    \textit{Unaproved wireless cameras} & Unapproved wireless cameras are a security breach.\\
    \hline
    \textit{Vulnerable wireless building controls} & Home automation devices with  by default unsecured configurations.\\
 %   Configuración de dispositivos de automatización casera con parámetros de comunicación inalámbrica por defecto. \\
    \hline
    \textit{Unapproved IoT Emitters}& Devices like thermostats or wireless sensors inside the buildings using Technologies like Zigbee or LoRa with long-range coverage.\\
     %  Dispositivos como termostatos o sensores en el interior de construcciones con interfaces inalámbricas mediante tecnologías como Zigbee o LORA con rangos de cobertura muy amplios.\\
    \hline
    \textit{Vulnerable building alarm systems} & 
    Security systems elements like door sensors, motion detectors can be sensitive to jammer attacks using software defined radios \\.
    
% Los sistemas de seguridad, como detectores de movimiento o sensores en puertas y ventanas pueden ser afectados por señales interferentes generadas mediante sistemas de radio definida por software de bajo costo.
%    \hline
    \end{tabular}
    \caption{Wireless vulnerabilities according to the Bastille Networks classification \cite{BastilleNetworksb}}
    \label{tab:bastille}
\end{table}

\subsection{SDR radios vulnerabilities}

The types of wireless attacks are varied, \cite{Moura2012} presents a classification of attacks targeting SDR tactical radios, while \cite{Fragkiadakis2013}, considers attacks with SDR radios within the Cognitive Radio Network Vulnerability Classification (CRNs). \cite{Soliman2018} analyzes the taxonomy of threats to cognitive radio networks by taking into account the layers of the OSI model for classification. Other studies focus specifically on the detailed analysis of a specific type of attack and/or vulnerability, such as \cite{Lichtman2016} where jamming-type attacks are analyzed.

The applicability of the reconfigurable radios concept has been proven in areas as demanding as tactical communications \cite{Moura2012}.However, there are technical factors such as power consumption, which restrict for their implementation to mobile devices. However, one of the vital aspects for their massification is to ensure that systems based on SDR technologies are protected against malicious codes \cite{Ulversoy2010}. 

The role of software-defined radio technology can be analyzed in several ways: firstly by considering the vulnerabilities of SDR radio platforms that can be exploited to affect their operation. A second approach arises from the use of SDR hardware for the generation of wireless attacks, which can affect the operation of various types of radio communication infrastructure, taking advantage of the vulnerabilities in protocols or technologies of the various radio ecosystems. The third aspect has to do with the potential of SDR technology for the development of diagnostic and control tools for cyber-threats and wireless cyber-attacks. 

Figure \ref{fig:ataques_c1} presents a classification of the types of wireless attacks targeting software-defined radios taking into account the work done by \cite{Moura2012}. The study considers vulnerabilities in tactical radios with software-defined radio technology. The authors present five different types of attacks: radiocontrol, personification, unauthorized data modifications, unauthorized data access and denial of service. Each of these typologies group a set of types of attacks and each of them arises from exploiting some vulnerabilities present in the system. Each of the elements of this structure is described in detail below.

\begin{figure*}[t]
        \centering
        \caption{Wireless attack classification, based on \cite{Moura2012}}
        \includegraphics[width=0.95\textwidth]{images/WAC_2.pdf}
        \label{fig:ataques_c1}
\end{figure*}

%\subsubsection{RADIOCONTROL}
%In this kind of attack the opponent achieves partial or total control of the radio by injecting malicious software (software injection attack) through the radio interface or physical access to the device, in order to compromise its operation. A software injection attack can exploit vulnerabilities such as buffer overflow, waveform download and start-up.
 
%\subsubsection*{Buffer overflow}
%Occurs by manipulating the amount of data stored in the radio buffer, exceeding its capacity and causing a malfunction of the device as explained by \cite{Al-SakibKhanPathan2016}. A software injection attack can exploit the vulnerabilities of the hardware with respect to the data management processes present in its input or output buffers. There are two kinds of vulnerabilities of this type: heap-based and stack-base. The former occurs when the buffer is located in an area of memory where the data is stored dynamically; while the later occurs when the buffer is located in the stack, which is a memory area where local data and return addresses of functions are stored.
 
%\subsubsection*{Waveform download} 
%In this type of software injection attack, the original waveform of the radio signal is modified. This occurs when an attacker exploits the vulnerability of the radio information download protocol, modifying the mechanisms that ensure the authenticity of the code, its integrity and version. This causes the radio to operate erratically, thereby affecting the quality of the communication service.

%\subsubsection*{Start-up} This vulnerability is present in manufacturing processes, where the malicious code can be embedded in a non-volatile memory used for initialization. The vulnerability is associated with the process of verifying the integrity of radio initialization routines.

%\subsubsection{SPOOFING}
%In such attacks, the purpose of the attacker is to deceive the radio by adopting a false identity that allows him to gain authorized access. The goal may be to impersonate a server, network or radio, or act in the midst of the interactions of the elements in the network. The attacker may also seek to acquire information, modify data that is sent, deceive the user, or modify SDR radio parameters. Attacks such as replay, authentication break and GPS spoofing fall in this category.

%\subsubsection*{Replay:} A signal can be recorded and then broadcasted via an SDR radio. This type of attack can be very effective on systems without authentication protocols.\cite{Uchikawa2002} analyzes a safe method for software downloads on FPGA-based SDR systems. 

%\textit{Krack} (\textit{Key Reinstallation attack}) is a replay attack aimed at WiFi networks with a WPA2 protocol. It was discovered in 2016 by researchers from the University of Leuven. Technical details can be found in \cite{Vanhoef2017}.It occurs in the negotiation process (4-way handshake) of the WPA2 protocol, during which the key to encrypt session traffic is generated. An attacker can access the information when the key is reused, since the WPA2 protocol does not guarantee that the key will be used only once. With this attack, it is not possible to know the key used to connect to the WiFi network, but it is possible to spy on all traffic.

%\subsubsection*{Authentication break:} This type of attack takes advantage of protocol failures in their authentication processes, thus enabling radio spoofing. Vulnerabilities have been identified in technologies such as IEEE 802.11 including WEP, WPA-PSK or EAP/LEAP.

%\subsubsection*{GPS Spoofing:} The signal received by a GPS can be supplanted so that the receiver can decode coordinates different from those of the actual position. A single transmitter or a set of them can perform the attack.

%\subsubsection{UNAUTHORIZED MODIFICATION OF DATA} 
%The attacker seeks to alter the data that is transmitted through variations to the waveform, changing parameters in the internal configuration of the device through modifications to the software or hardware.
 
%\subsubsection*{Software injection:} Includes modifications to data or radio parameters, internal protocols or system configuration files, data flow control processes. 

%\subsubsection*{Hardware Injection:} This type of attack can take advantage of processor hardware deficiencies or limitations to modify the radio's functioning. Furthermore, some vulnerabilities can be introduced into the hardware and function as a backdoor that can enable or disable hidden functions, known as a hardware Trojan, which poses a danger to electronic devices building processes used in critical infrastructure systems. \cite{Moein2016} characterizes the types of hardware Trojans for all phases of the construction cycle of an integrated circuit.  The authors present the design of a matrix for the evaluation of hardware trojans.  The U.S. Government's Advanced Research Projects Agency (DARPA) created the \textit{Trusted Integrated Circuits} \cite{DARPA}, to develop technologies to ensure reliability in the manufacturing processes of electronic devices used in military systems.\cite{Hasegawa2018} describes a method for detecting hardware Trojans by using Machine Learning classification techniques.

%\subsubsection{UNAUTHORIZED DATA ACCESS }
%This category includes the types of attacks that exploit software or hardware vulnerabilities to access information without necessarily modifying it.

%\subsubsection*{Hardware Injection}
%In this type of attack, radio hardware can be violated by installing data recording devices or sniffers. The operating parameters of the radio device are not necessarily modified, but copies of the firmware or information being transmitted or received are obtained.

%\subsubsection*{Software Injection}
%By installing malicious software, sensitive data, security keys or system information are accessed. The software could use the same SDR radio interface to send unauthorized data.

%\subsubsection*{Traffic analysis attacks} 
%This type of attack gains access to data traffic and through its analysis it is possible to determine aspects such as the identities of the transmitter and/or receiver, details of the protocols used, data patterns or the copy of the data flow. \cite{Feghhi2016} shows the analysis of this type of attack with tests carried out on both wireless and wired networks, reaching 90\% success rates. 

%\subsubsection*{Side-channel} 
%In this type of attack information is obtained from parameters such as variations in the electromagnetic behavior of the hardware or power consumption, and the attacker seeks to reconstruct the data of the source by means of statistical processing of the obtained signals. One of the most well-known attacks is known as TEMPEST, Telecommunications Electronics Material Protected from Emanating Spurious Transmissions, whereby information on a monitor can be reconstructed from the measurement of electromagnetic emissions from the device.\cite{Kuhn1998} presents an analysis on the functioning of this type of attack.

%\subsubsection*{Fault based}
%In this type of attack, hardware failures are introduced in order to modify its normal operation and seeks access to sensitive information.\cite{Pellegrini2010} describes an attack that alters the power voltage of the hardware to generate errors that allow obtaining a 1024-bit RSA key from Xilinx Virtex2Pro FPGA-based hardware. The attack algorithm was implemented on a Linux SPARC system.\cite{Mestiri2014}  describes the performance evaluation of the AES algorithm used in some embedded systems in the face of fault-based attack. The fault detection system was implemented in a Virtex-5 FPGA, achieving 99.86\% performance rate.

%\subsubsection*{Social Engineering} In this type of attack, people are manipulated for the purpose of obtaining confidential information or altering the functioning of a radio system. People can be impersonated to gain access to radio systems' operating areas to obtain information related to system security, or installation of storage hardware on radio communication systems.

%\subsubsection*{Eavesdropping}
%This type of attack seeks to listen to a communication without authorization. In wireless systems, this type of attack can be passive, when only listening to the communication, or active when interacting by sending some kind of request \cite{Dai2017}. En \cite{Liao2018} models a scenario for this type of attack in the context of IoT.

%\subsubsection{DENIAL OF SERVICE} 
%The purpose of this type of attack is to take the SDR device out of operation. Various types of radio vulnerabilities can be exploited when implementing this kind of attack.

%\subsubsection*{Jamming} It seeks to affect communication from and/or to another device by generating interference that affects the level of the signal to noise ratio. This type of attack can stop the flow of information from the radio system. \cite{Lichtman2016} describes the taxonomy of these types of attacks and the different techniques for their implementation.\cite{Patwardhan2014} presents a technique known as \textit{Jamming Beamforming}.

%\subsubsection*{Flooding}
%The attacker sends a large number of messages with a very high transmission rate seeking to render the radio unable to process them, generating a refusal in the communication service.

%https://datafloq.com/read/understanding-sdr-based-attacks-on-iot/3735



\subsection{IoT wireless ecosystem  vulnerbilities }
Table \ref{tab:ataques_iot} shows the classification of vulnerabilities of the Internet of Things according to a layer model described in \cite{Frustaci2018}.The three-level model considers: perception, transport and application. In the perception layer are physical IoT devices; various types of transducers obtain the data and devices are collected through wireless ecosystem technologies, such as those shown in Figure \ref{fig:ecosistema}. Generally, the devices used do not have high computing power due to limitations in power consumption or manufacturing costs.The transport layer is responsible for transmitting the information obtained in the perception layer to some of the processing systems, using access networks such as 3G, WiFi, ad hoc or the Internet. The application layer provides the services required by users. At this level, solutions such as smart-cities, smart-healthcare, etc are implemented. An application sublayer allows to manage all types of derivative services such as performing intelligent computing, implementing localization services, or serving as an interface with cloud computing systems. 

At each level, the authors identify a set of vulnerabilities. According to the analysis, it is considered that the level of perception is the least secure due to the physical exposure of IoT devices, hardware limitations and heterogeneity of technologies and where the following types of attacks can occur: physical, impersonation, denial of service ,and routing and data transit.
 
\begin{table}[ht!]
\small
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Layer} & \textbf{Vulnerability} \\ 
\midrule
\multirow{3}{*}{\textit{Application}} 
 & {Data jailbreak} \\
 & {Denial-of-service attacks} \\
 & {Malicious code injection } \\
 \hline
\multirow{3}{*}{\textit{Transport}} 
 & {Routing attacks} \\
 & {Denial-of-service attacks} \\
 & {Data transit attacks} \\
  \hline
\multirow{5}{*}{\textit{Perception}} 
 & {Physical attacks} \\
 & {Spoofing} \\
 & {Denial-of-service attacks} \\
 & {Routing attacks} \\
 & {Data transit attacks}\\
  \hline
\end{tabular}
\caption{\label{tab:ataques_iot}IoT Wireless Vulnerabilities, according to \cite{Frustaci2018}}
\end{table}

Perception layer attacks may be: physical, impersonation, denial of service, routing, and data traffic attacks.

%\subsubsection{PHYSICAL ATTACKS} Oriented to hardware components of the IoT system. Among them are:
%\subsubsection*{Nodes Manipulation:}The node, or any of its part thereof, can be altered, allowing access to or altering sensitive device and network information, in addition to the keys used in cryptography or routing tables.
%\subsubsection*{Malicious Code Injection:}The attacker physically introduces a malicious code, with the intention of gaining access to the IoT system.

%\subsubsection{SUPLANTATION} A malicious code alters the identity of a node, thereby taking advantage of the complexity of the authentication that a distributed system is subject to.
%\subsubsection{DENIAL OF SERVICE(DoS)} In this type of attack, the limited processing capacity of the nodes is exploited, thus affecting their operation.

%\subsubsection{ROUTING ATTACKS} Using intermediate nodes, routing paths can be modified during the data collection and forwarding process.

%\subsubsection{DATA TRANSIT ATTACKS} Related to confidentiality and integrity during data transit, attacks such as sniffing and/or man-in-the-middle may occur.

\subsection{Attacks on Cognitive radio networks}

Table  \ref{tab:ataques_cognitive} shows a classification for the types of attacks on cognitive radio networks according to the classification made by \cite{Fragkiadakis2013}. The vulnerabilities of cognitive radio systems relate to two of the main characteristics in this technology: its cognitive capacity and its reconfigurability. In the first case, attacks seek to emulate primary transmitters and/or transmit false observations of the spectrum sensing process. In the second scenario, by installing a malicious code, an attacker can take control of the radio. 

\begin{table}[ht!]
      \centering
       \begin{tabular} { m{8em} m{4em} m{12em} } 
      %\cols{lcl} 
       %\begin{tabular}{*{2}{llc}}
%      \begin{tabular}{*{10}{lllc}}
        \hline
       \textbf{Type of attack} & \textbf{Layer} & \textbf{Description }\\
        \hline
    % Emulación de usuario primario
     Primary user emulation & Physical & Signals emulation of primary transmitter \\
     %Emulación de señales de transmisión del usuario primario   
        \hline
     %Falsificación de los datos del sensado del espectro
     spectrum sensing data falsification ,(SSDF) \cite{Sharifi2016}  & Physical & Wrong observations concerning to spectrum sensing \\
     %ción errónea del estado del espectro   
        \hline   
    %Ataques al canal de control común
     Common control channel & Medium access  & Spoofing ,  congestion,jamming    \\
        \hline
    % Ataque por falsificación de \textit{beacon}
     Beacon falsitication & Medium access & Disruption of synchronization between IEEE 802.22 WRANs\\ 
    % Interrupción de la sincronización entre WRANs IEEE802.22    
          \hline
   Cross-Layer & All layers & Advanced attacks across multiple layers \\ %Ataques sofisticados que pueden involucrar varias capas \\
          \hline
     Software Defined Radio  & All layers & Manipulation of hardware and/or software on Software Defined Radios \\
    % Todo tipo de ataques producto de la manipulación de los radios SDR   
        \hline
        %*Producto descontinuado
        %\footnotetext{Descontinuado }
      \end{tabular}
      \caption{\label{tab:ataques_cognitive}Attacks on cognitive radio networks, based on \cite{Fragkiadakis2013}}
     
    \end{table}

Cognitive networks, by their nature, are also exposed to the vulnerabilities and attacks inherent to wireless networks and cognitive radios, for they are built using SDR radios and that makes them vulnerable to the same type of threats to which software-defined radio devices are exposed. 

\subsection{Cybersecurity experiences with SDR }

Table \ref{tab:ejemplos_SDR} presents a compendium of cases where SDR technology has been used to perform cybersecurity analyses on wireless technologies such as GSM, LTE, DECT, RFID, ACARS, ADS-B, LoRa, BLE, IEEE 802.11, IEEE 802.15.4, NFC or on communication systems with drones and vehicles; some of them are part of the wireless ecosystem of the Internet of things.The table specifies the type of SDR radio platform used and the type of attack or vulnerability implemented.

\begin{table*}[ht!]
%\tiny
\small
      \centering
       \begin{tabular} { m{17em} m{15em} m{10em} m{4em} } 
 %    \begin{tabular} { m{8em} m{5em} m{4em} m{4em} }    
       
      %\cols{lcl} 
       %\begin{tabular}{*{2}{llc}}
%      \begin{tabular}{*{10}{lllc}}
        \hline
       \textbf{Vulnerability, attack or analysis} & \textbf{Technology, objective} & \textbf{Hardware } & \textbf{References}\\
        \hline
       Spoofing & Drones & USRP & \cite{Nguyen}  \\
        \hline
       Spoofing & ACARS, FANS1/A & USRP B200 & \cite{Bresteau2018} \\
          \hline
       Spoofing & Vehicular Security (TMPS protocol) & USRP N210/ & \cite{Kilcoyne2016} \\
          \hline
       Spoofing & FM-based indoor localization. & USRP B100/WBX & \cite{Li2016} \\
          \hline
       GPS Spoofing & GNSS & USRP N210  & \cite{Schmidt2018} \\
          \hline
      % Spoofing & IoT  & Yard Stick & \cite{Talbot2018} \\
      %    \hline
       Man in the middle & IoT(Bluetooth 2.1)  & USRP 2 & \cite{Barnickel2012} \\
           \hline       
       Man in the middle & GSM & USRP B200 & \cite{Dubey2016} \cite{SantiagoAragonFedericoKuhlmann2015}  \\
            \hline
       IMSI catcher & GSM & USRP-N210/WBX USRP1& \cite{Hadzialic2014}
       \cite{Borgaonkar}
       \cite{Dabrowski2014} \\
          \hline
    %   IMSI catcher & GSM & USRP1 & \cite{Dabrowski2014} \\
    %      \hline
      Location leaks; denial of service & LTE & USRP B210 & \cite{Shaik2015} \\
          \hline
      Eavesdropping & ADS-B & RTL 2832U & \cite{TerrazasGonzalez2018} \\
          \hline 
      Eavesdropping & DECT  & USRP N210 RTL2832U & \cite{Sanchez2014} \\
          \hline
      Eavesdropping & Near Field Communication (NFC) & USRP N210  & \cite{Rong2016} \\
          \hline
      Protocols implementation & LoRaWan, BLE, IEEE802.11, IEEE802.15.4 & USRP E310 & \cite{Gavrila2018} \\
          \hline   
       TEMPEST  & Computer display & PXI-e 5665 USRP N210/WBX  & \cite{Elibol2012}
       \cite{Zhou2017} \\
          \hline 
      Side channel & Decryption AES-128 on 32 bits microcontroller & USRP2,RTL 2832U & \cite{Alakoca2017}
      \cite{Alakoca2016} \\
          \hline  
    %   TEMPEST, eavesdropping & Pantalla de computador & USRP N210/WBX & \cite{Zhou2017} \\
    %      \hline
      Penetration Testing & Tactical Radio Networks & HackRF One  & \cite{Heinaaro2015} \\
          \hline
      Replay & RFID & USRP N210/SBX  & \cite{Han2015} \\
          \hline   
      Jamming & OFDM & NI USRP 2921 & \cite{Alakoca2017}
      \cite{Alakoca2016} \\
          \hline 
    
      vulnerabilities analysis on physical layer & LTE & USRP N210 & \cite{Rao2017} \\
          \hline
      \end{tabular}
      \\
      \caption{\label{tab:ejemplos_SDR}Cases of attacks, vulnerabilities, or cybersecurity analysis with SDR technology }
     
    \end{table*}

\subsubsection{\textbf{Spoofing attacks}}
This type of attack is also known as man in the middle, and seeks to impersonate some of the elements in communication by taking advantage of the weaknesses that may exist in the protocols. Impersonated technologies may be highly varied.\cite{Nguyen} shows the development of a drone detection system by analyzing the characteristics of wireless signals.\cite{Bresteau2018} performs an analysis on aeronautical communications technology ACARS (Aircraft Communication Addressing and Reporting System) and FANS1/A (Future Air Navigation System, using USRP B200 radios to generate messages, seeking to assess the impact of this type of attack on air safety.\cite{Kilcoyne2016} assesses the vulnerability of wireless communication used in automatic air pressure measurement systems on the wheels of vehicles,  \textit{Tire Pressure Monitoring System}, a technology required by the \textit{National Highway Trafic Safety Administration} in the United States. A USRP N210 was used to capture, analyze and impersonate the signals.\cite{Li2016} designed an attack against an indoor location system based on frequency modulations using a USRP B100 and GNU Radio platform, in order to evaluate the system's vulnerabilities. \cite{Schmidt2018} explores methods for mitigating GNSS(\textit{Global Navigation Satellite System}) signage spoofing attacks using SDR radios and algorithms implemented in FPGAs.

Experiments concerning GSM technology vulnerability analysis are presented in  \cite{Dubey2016} and \cite{SantiagoAragonFedericoKuhlmann2015} where USRP radios such as B210 or N210 are used to impersonate a GSM base radio. \cite{Hadzialic2014}, \cite{Dabrowski2014} and \cite{Borgaonkar} show the implementation of an IMSI-catcher or stingray device using a USRP B210 radio and OpenBTS \cite{OpenBTS}.\cite{Shaik2015} describes vulnerability tests for LTE network access protocols using USRP B200 and OpenLTE radio \cite{Wojtowicz}. The results show two different types of vulnerabilities evaluated: the first one makes it is possible to obtain the precise location of a device using GPS coordinates or True range multilateration from the signal intensity reported by the cell. The second test showed the generation of a (DoS) attack targeting an LTE device.

\subsubsection{\textbf{Eavesdropping attacks}}
\cite{Rong2016}  introduces a method to prevent eavesdropping attacks on Near Field Communication (NFC) devices. It employs a USRP N210 radio to generate variable signals as to amplitude, frequency, or phase and introduces additional bits to prevent an attacker from identifying NFC message sequences.\cite{Sanchez2014} explains an attack against a communication system with Digital Enhanced Cordless Telecommunication technology (DECT, using USRP SDR radios and RTL-SDR  \cite{RTL-SDR.COM} operating in a frequency range from 1880 to 1930 MHz. The developed system enabled protocol analysis and recovery of G-encoded voice signals G726.\cite{TerrazasGonzalez2018} describes the ADS-B- aerial positioning signals-demodulation process (\textit{Automatic Dependent Surveillance Broadcast} using an SDR-RTL device. \cite{BastilleNetworksa} shows the vulnerability of various types of wireless keyboards and mouses that work with uncoded wireless technologies, thus exposing passwords, personal information, bank details, etc.\cite{MatthewKnight2016} describes the process of decoding and analyzing the LoRa technology protocol using a USRP B210 radio, GNU Radio and Python.

\subsubsection{\textbf{Sidechannel attacks}}

\cite{Zhou2017} describes a TEMPEST-type side-channel attack for the reconstruction of images from radio frequency signals captured by a log periodic antenna and an SDR-USRP radio platform.\cite{Kuhn1998} describes the physical principles of a TEMPEST attack, where imaging on a monitor is analyzed. \cite{Elibol2012} presents the results of reconstructing the images of various types of monitors, reaching a distance of 46 meters, using a directive antenna and the National Instruments PXi-E 5665 hardware. \cite{NoriyukiMiura2016} shows the development of a sensor that detects a variations of electromagnetic fields near processing devices for the purpose of detecting possible attacks.

\subsubsection{\textbf{Jamming attacks}}

\cite{Alakoca2017} analyzes the effects of a jamming attack targeting an OFDM communication system, and analyzes metrics such as BER, MER and EVM. In the implementation of the testbed, NI USRP 2921 radios were used.\cite{Alakoca2016} an OFDMA system was implemented using USRP NI 2921 radios that allowed to measure performance against jamming attacks. \cite{Patwardhan2014} describes a method to mitigate the effect of a jamming attack using beamformig techniques; USRP2 and GNU Radio radios were used in the proof of concept.

\subsection{SDR as a cybersecurity tool }

The potential of Software-defined radio technology as a tool for analysis in cybersecurity is very high, especially when considering its cognitive possibilities. Cybersecurity analysis requires the use of techniques to assess the vulnerability of systems using procedures framed within ethical hacking. One of the techniques, known as systems penetration tests or pentest, allows to establish if there are vulnerabilities or if the defenses of a system are enough. The results of these tests help improve network security. One of the most commonly used tools for these procedures is Kali-Linux \cite{Lisitsa2018};  which is Linux distribution that includes support for some SDR platforms such as RTL, HackRF, UHD hardware and Funcube. The technologies included in the tool are limited to Wi-Fi, Bluetooth and NFC.
In \cite{Picod2014a} the authors describe the tool for penetration testing Scapy, developed in Python language, which allows capturing, decoding and building packages for protocols such as 802.15.4, ZWave and Wireless M-Bus using a USRP B210 device. \cite{Heinaaro2015} describes a set of tests to identify vulnerabilities in military radio networks. SDR USRP and HackRF One devices are used as radio platforms. Bastille Networks \cite{BastilleNetworks} is a company engaged in identifying risks in what they call the “Internet of radios”. For the development of their cybersecurity audit services, they have developed and patented their own tools to diagnose or control cybersecurity threats: Collaborative Bandit Sensing; Bayesian Device Fingerprinting and Distributed Tomographic Localization.These tools were developed from software-defined radio devices.
\cite{Visoottiviseth2017} describes the PENTOS tool, designed to perform penetration testing on IoT devices, but limited to Wi-Fi and Bluettoth technologies.In \cite{Sagduyu2017} the authors describe the design and implementation of the EZPro software tool, which enables the testing and evaluation of tactical communications against jamming, PU Emulation, protocol emulation and SSDF (\textit{Spectrum Sensing Data Falsification}) attacks.











==> A Technical Review of Wireless security for the Internet of things_/5_overview_discussion.tex <==
Figure \ref{fig:ecosistema} shows the magnitude of the IoT wireless ecosystem, operating frequencies, and standards. It shows several emerging technologies based on the 802.15.4 standard, such as: Wi-sun (802.15.4e), Thread, ZigBee NAN, ISA100.11a, OnRamp, Wireless Hart, MiWi, Positive Train ctrl (802.15.4p) and 802.15.4m. Another set of emerging  WiFi-based technologies was identified, to wit, 802.11ac, 802.11ad, 802.11ah (HaLow), 802.11p (WAVE), 802.11af (Super Wi-Fi or WhiteFi). One of the major fields of development and competition among manufacturers is LPWA (Low Powe Wide Area) networks, where there are two large unlicensed LPWA groups that group technologies such as: LoRa, SigFox, Telensa and OnRamp, and a second LPWA-licensed group encompassing mobile technologies based on LTE and GSM such as NB-IoT and EC-GSM-IoT.

Table \ref{tab:ADC-DAC} shows the technical characteristics of the most common software-defined radio platforms, taking into account the number of bits used in ADC and DAC converters, their frequency ranges, transmission and/or reception capabilities and sampling rates. SDR technology has evolved thanks to the development of converter manufacturing techniques, moving from sampling rates in the order of 200 [Kb/s] used in 1999 to rates of 200 [MS/s] in devices manufactured in 2016. 

SDR hardware is in full development; recent platforms such as CRISOM  \cite{Pervices}  have ADC sampling rates of 370.16 [MS/s] and 2500,16 [MS/s] for DAC, plus an ARM Cortex-A9 MP processor and FPGA-Arria V ST SOC. Other SDR platform developments integrate processing capabilities for working with deeplearning techniques, such as the AIR-T (Artificial Intelligence Radio - Transceiver) platform composed of a 2x2 SDR MIMO system with a 256-core Jetson TX2 GPU. Improvements in conversion rates and increased computing power make it possible to process the large flow of I/Q samples and the implementation of modern wireless communications standards.

Several types of wireless system attacks and vulnerabilities were identified. Figure \ref{fig:ataques_c1} presents a classification of the types of wireless attacks for SDR radios. Table \ref{tab:bastille} describes the most common wireless vulnerabilities, according to the company Bastille Networs.Table \ref{tab:ataques_cognitive}, describes the types of attacks against cognitive radio networks.Table \ref{tab:ataques_iot} presents IoT's various wireless vulnerabilities according to a three-tier model proposed by \cite{Frustaci2018}. The literature identifies the perception level as the most vulnerable, exposed to physical, impersonation, and routing and data traffic attacks, due to limitations in hardware, physical exposure of devices and heterogeneity of technologies. One of the efforts to develop solutions related to improving manufacturing processes is the DARPA-funded  \textit{Trusted Integrated Circuits} for the design of technologies to ensure the reliability of hardware used in military systems.

The variety of SDR platforms is increasingly wide, as seen in table \ref{tab:ADC-DAC}, which has allowed to democratize knowledge in software-defined radio technology. Table \ref{tab:ejemplos_SDR} shows various implementation cases of wireless attacks using software-defined radio technology.The most commonly used radio platforms for this purpose are the USRP. Among the most common implementations are: spoofing, Eavesdropping, side channel, jamming, replay. The implementation of pentesting tools that show the potential of SDR technology for the development of cybersecurity tools was identified as well.

The research challenges related to the security of IoT Technologies are manifold, considering the heterogeneous characteristics of wireless technologies and the lack of standards for manufacturing secure IoT devices.

Future systems based on SDR radios have great advantages due to their flexibility to adapt to new communication technologies, but this very flexibility poses great risks. It is still unclear how to prevent software in radios from being modified or what strategies are most convenient for the protection of software and hardware of devices.

SDR platforms can operate in a frequency range from DC to 6 GHz, a range where there is a high percentage of current communication technologies and also have reasonable processing capabilities. However, the potential of the technology lies in the software being developed and the processing techniques implemented, wherefore it is important to consider that the design of solutions aimed at cybersecurity in wireless systems is a complex issue that involves areas of knowledge such as digital signal processing, communications systems, networks and communication protocols, signal propagation, antennas and microwave systems, among others.

Cyber security challenges for the Internet of Things are so complex that software-defined radio technology itself cannot be considered as a solution. SDR technology can be seen as a tool that can be combined with cognitive techniques and intelligent techniques such as deeplearning, which can be easily adapted to rapid technological changes.In this sense, the most ambitious initiative undergoing development is the DARPA \textit{Spectrum Collaboration Challenge} \cite{DARPAa}, a challenge designed to be carried out over a period of three years (2017-2019).It seeks to apply artificial intelligence techniques to expand the capabilities of software-defined radio technology. It uses the \textit{Colosseum} infrastructure, which is a laboratory built at the Applied Physics Laboratory (APL) at Johns Hopkins University, composed of 256 USRP radios and a set of servers with GPU processing capabilities.
